Can Community Notes Replace Professional Fact-Checkers?

Two commonly employed strategies to combat the rise of misinformation on social media are (i) fact-checking by professional organisations and (ii) community moderation by platform users. Policy changes by Twitter/X and, more recently, Meta, signal a shift away from partnerships with fact-checking organisations and towards an increased reliance on crowdsourced community notes. However, the extent and nature of dependencies between fact-checking and helpful community notes remain unclear. To address these questions, we use language models to annotate a large corpus of Twitter/X community notes with attributes such as topic, cited sources, and whether they refute claims tied to broader misinformation narratives. Our analysis reveals that community notes cite fact-checking sources up to five times more than previously reported. Fact-checking is especially crucial for notes on posts linked to broader narratives, which are twice as likely to reference fact-checking sources compared to other sources. Our results show that successful community moderation relies on professional fact-checking and highlight how citizen and professional fact-checking are deeply intertwined.

==> BigTables/countries.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{0.98\textwidth}{!}{%
    \fontsize{10}{10}\selectfont
    \sisetup{table-format = 3.2, group-minimum-digits=3}

\begin{tabular}{lll}
\toprule
Country &        Language &  Subreddits \\ 
\midrule
Australia      &     English &                           \subreddit{australia}, \subreddit{Australia\_}, \subreddit{australian}, \subreddit{sydney}, \subreddit{melbourne} \\
Brazil         &  Portuguese &                            \subreddit{brasil}, \subreddit{brasilivre}, \subreddit{GTAorBrazil}, \subreddit{brasilia}, \subreddit{saopaulo} \\
China          &     Chinese &                                                                       \subreddit{China}, \subreddit{China\_irl}, \subreddit{real\_China\_irl} \\
Colombia       &     Spanish &                                                                       \subreddit{Colombia}, \subreddit{ColombiaReddit}, \subreddit{Bogota} \\
Costa Rica     &     Spanish &                                                                                                   \subreddit{costarica}, \subreddit{Ticos} \\
Croatia        &    Croatian &                                                                                                    \subreddit{croatia}, \subreddit{zagreb} \\
Czech Republic &       Czech &                                                                                                                          \subreddit{czech} \\
Ecuador        &     Spanish &                                                                                                                        \subreddit{ecuador} \\
Estonia        &    Estonian &                                                                                                                          \subreddit{Eesti} \\
Faroe Islands  &         All &                                                                                                                   \subreddit{Faroeislands} \\
Finland        &     Finnish &                                                                                                                          \subreddit{Suomi} \\
France         &      French &                                                                                                      \subreddit{france}, \subreddit{paris} \\
Georgia        &    Georgian &                                                                                                \subreddit{Sakartvelo}, \subreddit{tbilisi} \\
Germany        &      German &                                                              \subreddit{de}, \subreddit{deuchland}, \subreddit{Munich}, \subreddit{berlin} \\
Ghana          &     English &                                                                                                                          \subreddit{ghana} \\
Greece         &       Greek &                                                                                                                         \subreddit{greece} \\
Hong Kong      &     Chinese &                                                                                                                       \subreddit{HongKong} \\
Iceland        &   Icelandic &                                                                                                                        \subreddit{Iceland} \\
India          &         All &                                          \subreddit{india}, \subreddit{IndiaSpeaks}, \subreddit{unitedstatesofindia}, \subreddit{askindia} \\
Indonesia      &  Indonesian &                                                                                                                      \subreddit{indonesia} \\
Israel         &      Hebrew &                                                                             \subreddit{Israel}, \subreddit{telaviv}, \subreddit{jerusalem} \\
Italy          &     Italian &                                                                                                      \subreddit{italy}, \subreddit{Italia} \\
Japan          &    Japanese &                                                                                 \subreddit{japan}, \subreddit{tokyo}, \subreddit{newsokur} \\
New Zealand    &     English &                                                                                               \subreddit{newzealand}, \subreddit{auckland} \\
Oman           &      Arabic &                                                                                                                           \subreddit{Oman} \\
Peru           &     Spanish &                                                                                                                           \subreddit{PERU} \\
Philippines    &     English &                                                                                                                    \subreddit{Philippines} \\
Poland         &      Polish &                                                                                                                         \subreddit{Polska} \\
Portugal       &  Portuguese &                                                                                \subreddit{portugal}, \subreddit{lisboa}, \subreddit{porto} \\
Romania        &    Romanian &                                      \subreddit{Romania}, \subreddit{bucuresti}, \subreddit{iasi}, \subreddit{cluj}, \subreddit{timisoara} \\
Serbia         &     Serbian &                                                                                                                         \subreddit{serbia} \\
Slovakia       &      Slovak &                                                                                                                       \subreddit{Slovakia} \\
South Africa   &         All &                                                                    \subreddit{southafrica}, \subreddit{capetown}, \subreddit{johannesburg} \\
South Korea    &      Korean &                                                                                                                         \subreddit{hanguk} \\
Spain          &     Spanish &                                                           \subreddit{Espana}, \subreddit{spain}, \subreddit{Madrid}, \subreddit{Barcelona} \\
Sweden         &     Swedish &                                                  \subreddit{Sverige}, \subreddit{sweden}, \subreddit{stockholm}, \subreddit{svenskpolitik} \\
Turkey         &     Turkish &                                                            \subreddit{Turkey}, \subreddit{istanbul}, \subreddit{ankara}, \subreddit{Ismir} \\
Ukraine        &   Ukrainian &                                                                                                \subreddit{ukraine}, \subreddit{Ukraine\_UA} \\
United Kingdom &         All &  \subreddit{unitedkingdom}, \subreddit{london}, \subreddit{manchester}, \subreddit{CasualUK}, \subreddit{unitedkingdom}, \subreddit{askuk} \\
USA            &         All &                                                                                                                      \texttt{All states subreddits} \\
Vietnam        &  Vietnamese &                                                                                                                        \subreddit{VietNam} \\
\bottomrule
\end{tabular}
}
    \caption{Countries, languages and subreddits used in the correlation study.}
    \label{tab:countries_data}
\end{table*}

==> BigTables/general_examples.tex <==
\begin{table*}

 \centering
 \resizebox{0.98\textwidth}{!}
 {%
 \fontsize{12}{12}\selectfont
 \sisetup{table-format = 3.2, group-minimum-digits=3}
 
 \begin{tabular}{p{12cm}cc}
 \toprule
 \textbf{Sentence}  & \textbf{Predicted Value} & \textbf{Predicted Stance} \\ 
 \midrule
The green party was literally removed from the ballot in key battleground states in the 2020 election. & Power & Negative \\
When you’re trained by a leader you become a leader. & Power & Positive \\
I've been learning jazz for about 8 months and still can't write a single good peace, is that normal?Just wondering if Im not deaf because every time I'm trying to write something I end up raging. In general I make music for 4-5 years if that matters. & Achievement & Negative \\
My first ever attempt at finger crochet (or any crochet for that matter)! I’m really proud of myself and just wanted to share somewhere :) & Achievement & Positive \\
I have never had a birthday celebrationSo my parents are Jehovah's witnesses I'm not but I have never received a birthday present and this year I'm really depressed I want to celebrate but I'm broke & Hedonism & Negative \\
To love more is Beautiful.I wish you Wonderful evening and happy weekend & Hedonism & Positive \\
This video gave me anxiety. It’s so inefficient with its movements that it made me squirm. & Stimulation & Negative \\
This awe inspiring film is the culmination of 3 months working underwater, diving, exploring and filming the most remote corners of the Great Barrier Reef. It showcases some of the most stunning scenes, schooling sharks and most vibrant coral reef the ocean has to offer. Hope you enjoy! & Stimulation & Positive \\
Having to lie so that you don't have to work Saturdays is funny and wholesome smh & Self-direction & Negative \\
If you want to be better at squatting, this is fine.  If you are going for a specific aesthetic, evaluate/critique your physique for any lagging parts areas, then choose the exercises that help bring them up. & Self-direction & Positive \\
"The only moral abortion is MY abortion" or "Grifters gonna Grift" & Universalism & Negative \\
I REALLY THINK ALL OF US HUMANS NEED TO BE REPRESENTED PROPERLY, REGARDLESS OF WHAT LANGUAGE PACKS WE HAVE INSTALLED. & Universalism & Positive \\
And then blaming the teacher when half the class fails. & Benevolence & Negative \\
please ban mentions of hasan off of LSF. his mental health is being affected by the harassment from this sub.	& Benevolence & Positive \\
Respect my religion while I shove it down your throat.... & Tradition & Negative \\
Korobeiniki: known in the West as "Tetris music"; in Russian, it\'s a folk song about courtship. & Tradition & Positive \\
There is a literal detailed police report of him beating the shit out of his then girlfriend.	& Conformity & Negative \\
Indian minister drinks dirty water from 'holy' river polluted with sewage to show locals it's safe... ends up in hospital days later & Conformity & Positive \\
This is in Mexico. The guy can literally pay the cops to look the other way, and he obviously has the money to do so & Security & Negative \\
India also built the largest border walls with pakistan, that too in the Himalayan foothills and thar desert. Really helped in curbing cross border terror though. & Security & Positive \\

 \bottomrule
 \end{tabular}
}
\caption{Examples of posts and comments from Reddit and the values and stances that the relevance and stance models predicted for each instance.}
\label{tab:posts_examples}
\end{table*}

==> BigTables/misclassificatioins.tex <==
\begin{table}

 \centering
 \resizebox{0.98\columnwidth}{!}
 {%
 \fontsize{8}{8}\selectfont
 \sisetup{table-format = 3.2, group-minimum-digits=3}
 
 \begin{tabular}{lp{4cm}p{1.5cm}}
 \toprule
 \textbf{Val} & \textbf{Sentence}  & \textbf{Annotated Average Rank} \\ 
 \midrule
SD & idk it brings some discussions to the community, can`t be bad & 2.33 \\
PO & You really gave it all you had very impressive content  & 2.66 \\
CO & Turkish guy debates Marxism and Freud with a street upper & 2.33 \\ 
BE & Claiming a fictional character has did because your coworker/psychologist said so based off of a movie & 2.33 \\
PO & What is each of your favorite song from Mercurial World to perform live? & 2.66 \\
 \bottomrule
 \end{tabular}
}

\caption{Instances where the relevance model predicted that the sentence expresses a value with high confidence (above 0.8), whereas the annotators concluded that the sentence does not express the value.}
\label{tab:rel_misclassification}
\end{table}


\begin{table}

 \centering
 \resizebox{0.98\columnwidth}{!}
 {%
 \fontsize{8}{8}\selectfont
 \sisetup{table-format = 3.2, group-minimum-digits=3}
 
 \begin{tabular}{lp{4cm}p{1.5cm}}
 \toprule
 \textbf{Val} & \textbf{Sentence}  & \textbf{Predicted (wrong) Stance} \\ 
 \midrule
PO & Crypto traders using the war to make money. This is a new low & Pos \\
HE & God forbid you pay someone for their content that you enjoy.  & Neg \\
CO &SLPT: drive at speed in reverse gear through speed cameras to get fines repaid by the police & Pos \\ 
SD & If the island keeps drifting, the UK would be part of the US again? & Neg \\
UN &The double standards of western media towards third world countries & Pos \\
SD & The coffee is probably making it worse. People forget it’s a drug with consequences. & Neg \\
 \bottomrule
 \end{tabular}
}

\caption{Instances where the stance model misclassified a sentence.}
\label{tab:stance_misclassification}
\end{table}

==> BigTables/schwartz_values.tex <==



\begin{table*}[ht]
    \centering
    
    \fontsize{8}{9}\selectfont
    % \sisetup{table-format = 3.2, group-minimum-digits=3}
\begin{tabular}{lp{13cm}}
\toprule
Value & Description \\
\midrule

\schwartzvalue{Power}	& Social status and prestige, control or dominance over people and resources \\
\schwartzvalue{Achievement}	& Personal success through demonstrating competence according to social standards. \\
\schwartzvalue{Hedonism} &	Pleasure and sensuous gratification for oneself. \\
\schwartzvalue{Stimulation} &	Excitement, novelty, and challenge in life. \\
\schwartzvalue{Self-direction} &	Independent thought and action-choosing, creating, exploring. \\
\schwartzvalue{Universalism}	& Understanding, appreciation, tolerance, and protection for the welfare of all people and for nature. \\
\schwartzvalue{Benevolence}	& Preservation and enhancement of the welfare of people with whom one is in frequent personal contact. \\
\schwartzvalue{Tradition}	& Respect, commitment, and acceptance of the customs and ideas that traditional culture or religion provide. \\
\schwartzvalue{Conformity} &	Restraint of actions, inclinations, and impulses likely to upset or harm others and violate social expectations or norms. \\
\schwartzvalue{Security} &	Safety, harmony, and stability of society, of relationships, and of self. \\
\bottomrule

\end{tabular}
    \caption{The ten Schwartz values and their meaning; descriptions from \citet{schwartz-1994-universal}}\label{tab:value_description}
\end{table*}


==> BigTables/strong_signal.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{0.98\textwidth}{!}{%
    \fontsize{8}{8}\selectfont
    \sisetup{table-format = 3.2, group-minimum-digits=3}
    % \sisetup{table-format = 3.2, group-minimum-digits=3}
\begin{tabular}{lp{14cm}}
\toprule
Value & Subreddits \\
\midrule
%achievement    &   GED, CompTIA, AWSCertifications, EngineeringResumes, study, AzureCertification, GetStudying, cissp, findapath, learnprogramming, WGU\_CompSci, pmp, resumes, ADHD\_Programmers, dataanalysis, language\_exchange, PassNclex, PhD, C25K, technicalwriting \\
Tradition      & \subredditnegative{religion}, \subreddit{Anglicanism}, \subreddit{TraditionalCatholics}, \subreddit{AskAChristian}, \subredditnegative{AcademicBiblical}, \subreddit{Catholic}, \subreddit{AskBibleScholars}, \subreddit{Episcopalian}, \subredditpositive{AskAPriest}, \subredditnegative{Antitheism}, \subreddit{OrthodoxChristianity}, \subreddit{Catholicism}, \subredditnegative{antitheistcheesecake}, \subredditnegative{agnostic}, \subredditnegative{atheistmemes}, \subreddit{CatholicMemes}, \subredditpositive{Bible}, \subredditnegative{RadicalChristianity}, \subredditnegative{atheism}, \subredditnegative{religiousfruitcake}, \subredditnegative{Gnostic}, \subreddit{Christianity}, \subreddit{christianmemes}, \subreddit{OpenChristian}, \subredditnegative{paganism}, \subredditnegative{excatholic}, \subredditnegative{atheismindia}, \subredditnegative{EXHINDU}, \subreddit{ChristianUniversalism}, \subreddit{bahai} \\ \midrule
Benevolence    &  \subredditpositive{coparenting}, \subreddit{Stepmom}, \subreddit{BipolarSOs}, \subreddit{theotherwoman}, \subreddit{stepparents}, \subreddit{AdultChildren}, \subreddit{ADHD\_partners}, \subredditpositive{CaregiverSupport}, \subreddit{SingleParents}, \subredditpositive{Petloss}, \subredditpositive{Adoption}, \subreddit{emotionalabuse}, \subreddit{EstrangedAdultChild}, \subredditpositive{AgingParents}, \subreddit{FriendshipAdvice}, \subreddit{AnxiousAttachment}, \subreddit{Adopted}, \subreddit{attachment\_theory}, \subreddit{AsOneAfterInfidelity}, \subreddit{NarcAbuseAndDivorce}, \subreddit{regretfulparents}, \subreddit{survivinginfidelity}, \subredditpositive{Fosterparents}, \subreddit{AvoidantAttachment}, \subreddit{AlAnon}, \subreddit{Custody}, \subredditnegative{BPDlovedones}, \subreddit{Codependency}, \subreddit{emotionalneglect}, \subredditpositive{SuicideBereavement} \\ \midrule
Conformity     &                                                                  \subredditnegative{AgainstHateSubreddits}, \subredditnegative{reclassified}, \subredditnegative{TheseFuckingAccounts}, \subredditnegative{AmIFreeToGo}, \subredditnegative{ModSupport}, \subredditnegative{modsbeingdicks}, \subredditnegative{ModsAreKillingReddit}, \subredditnegative{policebrutality}, \subredditnegative{modhelp}, \subredditnegative{WatchRedditDie}, \subredditnegative{Bad\_Cop\_No\_Donut}, \subredditnegative{Chiraqhits}, \subredditnegative{JustUnsubbed}, \subredditnegative{legaladviceofftopic}, \subredditnegative{circlebroke2}, \subreddit{HOA}, \subredditnegative{BadNeighbors}, \subredditnegative{redditrequest}, \subredditnegative{law}, \subredditnegative{fuckHOA}, \subredditnegative{40kOrkScience}, \subredditnegative{legaladvice}, \subredditnegative{LegalAdviceIndia}, \subredditnegative{ACAB}, \subreddit{Ask\_Lawyers}, \subreddit{legaladvicecanada}, \subredditnegative{CapitolConsequences}, \subredditnegative{supremecourt}, \subredditnegative{NarcAbuseAndDivorce}, \subredditnegative{JustNoTruth} \\ \midrule
Hedonism       &                                                                                                      \subredditpositive{crossdressing}, \subredditpositive{transadorable}, \subredditpositive{Autumn}, \subredditpositive{TheMidnight}, \subredditpositive{dykesgonemild}, \subredditpositive{cakedecorating}, \subredditpositive{FreeCompliments}, \subredditpositive{GothStyle}, \subredditpositive{NailArt}, \subredditpositive{cozy}, \subredditpositive{PlusSizeFashion}, \subredditpositive{MTFSelfieTrain}, \subredditpositive{oldhagfashion}, \subredditpositive{femboy}, \subredditpositive{transpositive}, \subredditpositive{christmas}, \subredditpositive{malepolish}, \subredditpositive{RainbowEverything}, \subredditpositive{gaybrosgonemild}, \subredditpositive{HappyTrees}, \subredditpositive{selfie}, \subredditpositive{cookiedecorating}, \subredditpositive{weddingdress}, \subredditpositive{genderfluid}, \subredditpositive{happy}, \subredditpositive{Watercolor}, \subredditpositive{AltJ}, \subredditpositive{AnyaTaylorJoy}, \subredditpositive{BigNoseLadies}, \subredditpositive{Madonna} \\ \midrule
Power          &                                                                                              \subredditpositive{FundRise}, \subredditpositive{AskEconomics}, \subredditpositive{finance}, \subredditpositive{acorns}, \subredditpositive{HistoricalWhatIf}, \subredditpositive{geopolitics}, \subredditpositive{strongblock}, \subredditpositive{UWMCShareholders}, \subredditpositive{debtfree}, \subredditpositive{qyldgang}, \subredditpositive{rocketpool}, \subredditpositive{Anchor}, \subredditpositive{IndianStreetBets}, \subredditpositive{Economics}, \subredditpositive{dividends}, \subredditpositive{VoteBlue}, \subredditpositive{EuropeanFederalists}, \subredditpositive{defi}, \subredditpositive{ValueInvesting}, \subredditpositive{AlibabaStock}, \subredditpositive{CredibleDefense}, \subredditpositive{Stellar}, \subredditpositive{DalalStreetTalks}, \subredditpositive{CapitalismVSocialism}, \subredditpositive{PoliticalDiscussion}, \subredditpositive{LETFs}, \subredditpositive{suzerain}, \subredditpositive{AllCryptoBets}, \subredditpositive{SatoshiBets}, \subredditpositive{startups} \\ \midrule
Achievement    &                                                                                                              \subredditpositive{passive\_income}, \subredditpositive{FundRise}, \subredditpositive{ValueInvesting}, \subredditpositive{OptionsMillionaire}, \subredditpositive{EngineeringResumes}, \subredditpositive{xboxachievements}, \subredditpositive{algotrading}, \subredditpositive{FuturesTrading}, \subredditpositive{resumes}, \subredditpositive{abmlstock}, \subredditpositive{AllCryptoBets}, \subredditpositive{cryptostreetbets}, \subredditpositive{dividends}, \subredditpositive{SatoshiBets}, \subredditpositive{Forex}, \subredditpositive{EANHLfranchise}, \subredditpositive{IndianStockMarket}, \subredditpositive{quant}, \subredditpositive{Blogging}, \subredditpositive{aabbstock}, \subredditpositive{CryptoMars}, \subredditpositive{Daytrading}, \subredditpositive{ETFs}, \subredditpositive{startups}, \subredditpositive{SEO}, \subredditpositive{SaaS}, \subredditpositive{biotech}, \subredditpositive{SecurityAnalysis}, \subredditpositive{Wishstock}, \subredditpositive{Xelastock} \\ \midrule
Self-direction &  \subredditpositive{CapitalismVSocialism}, \subredditpositive{ScientificNutrition}, \subredditpositive{Abortiondebate}, \subredditpositive{DebateAnarchism}, \subredditpositive{BasicIncome}, \subredditpositive{DebateAVegan}, \subredditpositive{Neuropsychology}, \subredditpositive{changemyview}, \subredditpositive{AskEconomics}, \subredditpositive{AskPsychiatry}, \subredditpositive{AskDID}, \subredditpositive{nutrition}, \subredditpositive{AskSocialScience}, \subredditpositive{healthcare}, \subredditpositive{askpsychology}, \subredditpositive{radicalmentalhealth}, \subredditpositive{ketoscience}, \subredditpositive{DebateReligion}, \subredditpositive{Marxism}, \subredditpositive{PsychedelicTherapy}, \subredditpositive{psychoanalysis}, \subredditpositive{intentionalcommunity}, \subreddit{TrueUnpopularOpinion}, \subredditpositive{HealthInsurance}, \subredditpositive{Microbiome}, \subredditpositive{AskLibertarians}, \subredditpositive{sorceryofthespectacle}, \subredditpositive{actual\_detrans}, \subredditpositive{ScienceBasedParenting}, \subredditpositive{DebateAChristian} \\ \midrule
Universalism   &            \subredditpositive{DebateAVegan}, \subredditpositive{IsraelPalestine}, \subredditpositive{DebateEvolution}, \subredditpositive{DebateAnarchism}, \subredditpositive{DebateReligion}, \subredditpositive{changemyview}, \subredditpositive{Abortiondebate}, \subredditpositive{CapitalismVSocialism}, \subredditpositive{AskSocialScience}, \subreddit{EndlessWar}, \subredditpositive{LeftWingMaleAdvocates}, \subredditpositive{DebateAnAtheist}, \subredditpositive{TrueUnpopularOpinion}, \subredditpositive{PoliticalDiscussion}, \subredditpositive{Ask\_Politics}, \subredditpositive{IntellectualDarkWeb}, \subredditpositive{chomsky}, \subredditpositive{AskFeminists}, \subredditpositive{Marxism}, \subredditpositive{DebateCommunism}, \subreddit{israelexposed}, \subredditpositive{DebateAChristian}, \subredditpositive{AskAnthropology}, \subredditpositive{ControversialOpinions}, \subredditpositive{media\_criticism}, \subredditpositive{askphilosophy}, \subredditpositive{Socialism\_101}, \subredditpositive{climatechange}, \subredditpositive{conservation}, \subreddit{honesttransgender} \\ \midrule
Stimulation    &                                                                                          \subredditpositive{Autumn}, \subredditpositive{crossdressing}, \subredditpositive{TheMidnight}, \subredditpositive{transadorable}, \subredditpositive{FreeCompliments}, \subredditpositive{dykesgonemild}, \subredditpositive{cakedecorating}, \subredditpositive{xboxachievements}, \subredditpositive{PlusSizeFashion}, \subredditpositive{GothStyle}, \subredditpositive{cozy}, \subredditpositive{MTFSelfieTrain}, \subredditpositive{christmas}, \subredditpositive{AltJ}, \subredditpositive{Madonna}, \subredditpositive{weddingdress}, \subredditpositive{NailArt}, \subredditpositive{transpositive}, \subredditpositive{happy}, \subredditpositive{Hobbies}, \subredditpositive{HappyTrees}, \subredditpositive{BigNoseLadies}, \subredditpositive{oldhagfashion}, \subredditpositive{selfie}, \subredditpositive{gaybrosgonemild}, \subredditpositive{RainbowEverything}, \subredditpositive{BeachHouse}, \subredditpositive{RoomieOfficial}, \subredditpositive{Watercolor}, \subredditpositive{FlorenceAndTheMachine} \\\midrule
Security       &                                                       \subredditpositive{CredibleDefense}, \subredditpositive{ww3}, \subredditpositive{syriancivilwar}, \subredditpositive{geopolitics}, \subredditpositive{EndlessWar}, \subredditpositive{warinukraine}, \subredditpositive{AfghanConflict}, \subredditpositive{UkrainianConflict}, \subredditpositive{UkraineConflict}, \subredditpositive{CombatFootage}, \subredditpositive{LessCredibleDefence}, \subreddit{GunsAreCool}, \subredditpositive{war}, \subredditpositive{FutureWhatIf}, \subredditpositive{nuclearweapons}, \subredditpositive{WarCollege}, \subredditpositive{UkraineInvasionVideos}, \subredditpositive{UkraineRussiaReport}, \subredditpositive{RussiaUkraineWar2022}, \subredditpositive{UkraineWarReports}, \subredditpositive{N\_N\_N}, \subredditpositive{UkraineWarVideoReport}, \subredditpositive{HistoryWhatIf}, \subredditpositive{worldevents}, \subredditpositive{ukraine}, \subredditpositive{chomsky}, \subredditpositive{HistoricalWhatIf}, \subredditpositive{ukraina}, \subredditpositive{anonymous}, \subredditpositive{IndianDefense} \\
\bottomrule

\end{tabular}
}
    \caption{Subreddits with the highest signal for each one of the ten Schwartz values. The stance of \textcolor{OliveGreen}{Green} subreddits towards the value is positive (above $0.2$), whereas \textcolor{BrickRed}{Red} indicates negative stance (below $-0.2)$.}
    \label{tab:strongest_signal}
\end{table*}


% \begin{table*}[ht]
%     \centering
%     \fontsize{10}{10}\selectfont
%     % \sisetup{table-format = 3.2, group-minimum-digits=3}
% \begin{tabular}{p{2cm}p{13cm}}
% \toprule
% Value & Subreddits \\
% \midrule
% Achievement    &   \subreddit{study}, \subreddit{resumes}, \subreddit{PhD}  \\
% Benevolence    &             \subreddit{AmItheAsshole}, \subreddit{motherinlawsfromhell}, \subreddit{family}  \\
% Conformity     &                    \subreddit{Anger}, \subreddit{confession}, \subreddit{pettyrevenge}, \\ 
% Hedonism       &  \subreddit{happyrelationships}, \subreddit{sex}, \subreddit{depression} \\
% Power          &                                  \subreddit{FinancialPlanning},  \subreddit{smallbusiness}, \subreddit{GamblingAddiction}\\
% Security       &   \subreddit{foreignpolicy}, \subreddit{warinukraine}, \subreddit{CombatFootage} \\
% Self-direction &                  \subreddit{antidepressants} \subreddit{AnorexiaRecovery}, \subreddit{sugarfree}, 
% \subreddit{Allergies} \\
% Stimulation    & \subreddit{ShouldIbuythisgame}, \subreddit{socialanxiety}, \subreddit{MakeNewFriendsHere}, \subreddit{FreeCompliments} \\
% Tradition      & \subreddit{PrayerRequests}, \subreddit{Christians}, \subreddit{Anglicanism} \\
% Universalism   &  
% \subreddit{mixedrace}, 
% \subreddit{IsraelPalestine}, \subreddit{conservation},
% \subreddit{LGBTnews} \\
% \bottomrule

% \end{tabular}  
%     \caption{Subreddits with the highest signal for each of the ten Schwartz values.
% }
% \end{table*}

==> BigTables/strongest_stances.tex <==
\begin{table*}
    \centering
    \resizebox{0.98\textwidth}{!}{%
    \fontsize{8}{8}\selectfont
    \sisetup{table-format = 3.2, group-minimum-digits=3}

\begin{tabular}{lp{6cm}|p{6cm}}
\toprule
  Value & Positive Stance & Negative Stance \\ \midrule
Tradition & \subreddit{Ankrofficial}, \subreddit{lds}, \subreddit{CharliDamelioMommy}, \subreddit{Christian}, \subreddit{AskAPriest}, \subreddit{Bible}, \subreddit{bahai}, \subreddit{Quakers}, \subreddit{PrismaticLightChurch}, \subreddit{OrthodoxChristianity} & \subreddit{SuperModelIndia}, \subreddit{Jewdank}, \subreddit{EXHINDU}, \subreddit{DesiMeta}, \subreddit{linguisticshumor}, \subreddit{exmuslim}, \subreddit{AsABlackMan}, \subreddit{Satan}, \subreddit{IndoEuropean}, \subreddit{AfterTheEndFanFork} \\ \midrule
Benevolence & \subreddit{freebsd}, \subreddit{RandomKindness}, \subreddit{Terraform}, \subreddit{Petloss}, \subreddit{nextjs}, \subreddit{Wetshaving}, \subreddit{AllCryptoBets}, \subreddit{NixOS}, \subreddit{vancouverhiking}, \subreddit{ansible} & \subreddit{FromDuvalToDade}, \subreddit{CrimeInTheD}, \subreddit{NBAYoungboy}, \subreddit{40kOrkScience}, \subreddit{LILUZIVERTLEAKS}, \subreddit{DuvalCounty}, \subreddit{Phillyscoreboard}, \subreddit{Chiraqhits}, \subreddit{SummrsXo}, \subreddit{CARTILEAKS} \\ \midrule
Conformity & \subreddit{Ankrofficial}, \subreddit{nanotrade}, \subreddit{NervosNetwork}, \subreddit{Vechain}, \subreddit{steroids}, \subreddit{USCIS}, \subreddit{treelaw}, \subreddit{Stellar}, \subreddit{cancun}, \subreddit{JapanFinance} & \subreddit{Animewallpaper}, \subreddit{kencarson}, \subreddit{FromDuvalToDade}, \subreddit{LilDurk}, \subreddit{Cookierun}, \subreddit{freddiegibbs}, \subreddit{SummrsXo}, \subreddit{DestroyLonely}, \subreddit{Gunna}, \subreddit{okbuddydaylight} \\ \midrule
Hedonism & \subreddit{eastside}, \subreddit{RedditPHCyclingClub}, \subreddit{OaklandFood}, \subreddit{carcamping}, \subreddit{CryptoMars}, \subreddit{VeganBaking}, \subreddit{TheHague}, \subreddit{ZZZ\_Official}, \subreddit{pottedcats}, \subreddit{ambientmusic} & \subreddit{depression}, \subreddit{TIHI}, \subreddit{Shark\_Park}, \subreddit{willowbramley}, \subreddit{Phillyscoreboard}, \subreddit{migraine}, \subreddit{BodyDysmorphia}, \subreddit{SuicideWatch}, \subreddit{2meirl4meirl}, \subreddit{anhedonia} \\ \midrule
Power & \subreddit{Yotsubros}, \subreddit{Fitness}, \subreddit{CryptoMoonShots}, \subreddit{infertility}, \subreddit{AllCryptoBets}, \subreddit{ketoscience}, \subreddit{steroids}, \subreddit{ProgrammingLanguages}, \subreddit{cryptostreetbets}, \subreddit{cooperatives} & \subreddit{masterhacker}, \subreddit{Stake}, \subreddit{uknews}, \subreddit{RustConsole}, \subreddit{uspolitics}, \subreddit{OPBR}, \subreddit{BidenIsNotMyPresident}, \subreddit{capitalism\_in\_decay}, \subreddit{Patriot911}, \subreddit{occupywallstreet} \\ \midrule
Achievement & \subreddit{infertility}, \subreddit{theravada}, \subreddit{edrums}, \subreddit{raisingkids}, \subreddit{CryptoMars}, \subreddit{Yotsubros}, \subreddit{cozy}, \subreddit{gaidhlig}, \subreddit{PrismaticLightChurch}, \subreddit{learnrust} & \subreddit{DreamStanCringe}, \subreddit{FGOmemes}, \subreddit{AntiTrumpAlliance}, \subreddit{BidenWatch}, \subreddit{misanthropy}, \subreddit{Patriot911}, \subreddit{TRUTHsocialWatch}, \subreddit{Instagram}, \subreddit{TwitterCringe}, \subreddit{Negareddit} \\ \midrule
Self-direction & \subreddit{Mosses}, \subreddit{jungle}, \subreddit{LandscapingTips}, \subreddit{icecreamery}, \subreddit{esp32}, \subreddit{SatoshiBets}, \subreddit{rust\_gamedev}, \subreddit{openstreetmap}, \subreddit{QuantumComputing}, \subreddit{cryptostreetbets} & \subreddit{Negareddit}, \subreddit{misanthropy}, \subreddit{PeopleFuckingDying}, \subreddit{BoomersBeingFools}, \subreddit{AmericanFascism2020}, \subreddit{RepublicanValues}, \subreddit{FoxFiction}, \subreddit{ParlerWatch}, \subreddit{libsofreddit}, \subreddit{FragileWhiteRedditor} \\ \midrule
Universalism & \subreddit{SatoshiBets}, \subreddit{CryptoMars}, \subreddit{AllCryptoBets}, \subreddit{nextjs}, \subreddit{AskAstrophotography}, \subreddit{GardenWild}, \subreddit{vancouverhiking}, \subreddit{dungeondraft}, \subreddit{EatCheapAndVegan}, \subreddit{GraphicsProgramming} & \subreddit{CrimeInTheD}, \subreddit{FromDuvalToDade}, \subreddit{Phillyscoreboard}, \subreddit{DaDumbWay}, \subreddit{DuvalCounty}, \subreddit{Chiraqhits}, \subreddit{BruceDropEmOff}, \subreddit{punchableface}, \subreddit{ConservativeRap}, \subreddit{NYStateOfMind} \\ \midrule
Stimulation & \subreddit{CryptoMars}, \subreddit{cryptostreetbets}, \subreddit{JoshuaTree}, \subreddit{wonderdraft}, \subreddit{reenactors}, \subreddit{AllCryptoBets}, \subreddit{estoration}, \subreddit{yerbamate}, \subreddit{GiftIdeas}, \subreddit{OaklandFood} & \subreddit{depression}, \subreddit{Shark\_Park}, \subreddit{heck}, \subreddit{TwitterCringe}, \subreddit{depressed}, \subreddit{CommercialsIHate}, \subreddit{Demps}, \subreddit{D\_Demps}, \subreddit{christenwhitmansnark}, \subreddit{Sleepparalysis} \\ \midrule
Security & \subreddit{BoringCompany}, \subreddit{haskell}, \subreddit{ProgrammingLanguages}, \subreddit{rust}, \subreddit{psychoanalysis}, \subreddit{crypto}, \subreddit{steroids}, \subreddit{AskComputerScience}, \subreddit{infertility}, \subreddit{DebateEvolution} & \subreddit{holdmycosmo}, \subreddit{davidbowiecirclejerk}, \subreddit{RoastMyCat}, \subreddit{Chiraqhits}, \subreddit{DaDumbWay}, \subreddit{okbuddydaylight}, \subreddit{bottomgear}, \subreddit{SuicideWatch}, \subreddit{CrimeInTheD}, \subreddit{Bombing} \\ 
\bottomrule
\end{tabular}
}
\caption{Subreddits expressing each value's strongest positive and negative stances.}
\label{tab:strongest_stances}
\end{table*}

